FlyKD: Graph Knowledge Distillation on the Fly with Curriculum Learning

Knowledge Distillation (KD) aims to transfer a more capable teacher model's knowledge to a lighter student model in order to improve the efficiency of the model, making it faster and more deployable. However, the student model's optimization process over the noisy pseudo labels (generated by the teacher model) is tricky and the amount of pseudo labels one can generate is limited due to Out of Memory (OOM) error. In this paper, we propose FlyKD (Knowledge Distillation on the Fly) which enables the generation of virtually unlimited number of pseudo labels, coupled with Curriculum Learning that greatly alleviates the optimization process over the noisy pseudo labels. Empirically, we observe that FlyKD outperforms vanilla KD and the renown Local Structure Preserving Graph Convolutional Network (LSPGCN). Lastly, with the success of Curriculum Learning, we shed light on a new research direction of improving optimization over noisy pseudo labels.

==> table/sometab1.tex <==
\centering
\begin{tabular}{lll}
\toprule
\multicolumn{2}{c}{Part}                   \\
\cmidrule(r){1-2}
Name     & Description     & Size ($\mu$m) \\
\midrule
Dendrite & Input terminal  & $\sim$100     \\
Axon     & Output terminal & $\sim$10      \\
Soma     & Cell body       & up to $10^6$  \\
\bottomrule
\end{tabular}

==> table/sometab2.tex <==
\centering
\begin{tabular}{l|lcccccc}
\toprule
Method & Modality & Edit distance & BLEU & METEOR & Precision & Recall & F1 \\ \midrule
PDF                  & All      & 0.255 & 65.8 & 82.1 & 77.1 & 81.4 & 79.2 \\ \hline
GROBID               & All      & 0.312 & 55.6 & 71.9 & 74.0 & 72.1 & 73.0 \\ \cline{2-8}
                     &Tables    & 0.626 & 25.1 & 64.5 & 61.4 & 80.7 & 69.7 \\
+ LaTeX OCR %
                     & Plain text &0.363 & 57.4 & 69.2 & 82.1 & 70.5 & 75.9 \\
                     & Math     & 0.727 & 0.3 & 5.0 & 11.0 & 8.6 & 9.7 \\ \hline
\multirow{4}{*}{Nougat base (350M$^\ast$)} & All & \bf 0.071 & \bf 89.1 & \bf 93.0 & 93.5 & \bf 92.8 & \bf 93.1 \\ \cline{2-8}
                     & Tables     & 0.211 & 69.7 & 79.1 & 75.4 & 80.7 & 78.0 \\ 
                     & Plain text & 0.058         & 91.2 & 94.6   & 96.2      & 95.3   & 95.7 \\
                     & Math       & 0.128         & 56.9 & 75.4   & 76.5      & 76.6   & 76.5 \\ \bottomrule
\end{tabular}
